NetworkGym: Reinforcement Learning Environments for Multi-Access Traffic Management in Network Simulation

Mobile devices such as smartphones, laptops, and tablets can often connect to multiple access networks (e.g., Wi-Fi, LTE, and 5G) simultaneously. Recent advancements facilitate seamless integration of these connections below the transport layer, enhancing the experience for apps that lack inherent multi-path support. This optimization hinges on dynamically determining the traffic distribution across networks for each device, a process referred to as \textit{multi-access traffic splitting}. This paper introduces \textit{NetworkGym}, a high-fidelity network environment simulator that facilitates generating multiple network traffic flows and multi-access traffic splitting. This simulator facilitates training and evaluating different RL-based solutions for the multi-access traffic splitting problem. Our initial explorations demonstrate that the majority of existing state-of-the-art offline RL algorithms (e.g. CQL) fail to outperform certain hand-crafted heuristic policies on average. This illustrates the urgent need to evaluate offline RL algorithms against a broader range of benchmarks, rather than relying solely on popular ones such as D4RL. We also propose an extension to the TD3+BC algorithm, named Pessimistic TD3 (PTD3), and demonstrate that it outperforms many state-of-the-art offline RL algorithms. PTD3's behavioral constraint mechanism, which relies on value-function pessimism, is theoretically motivated and relatively simple to implement.

==> sections/td3_bc.tex <==
\section{TD3+BC}

\mh{Do we need this section anymore?}

We reproduce the TD3+BC algorithm from Fujimoto et al. in Algorithm 2.
Note that we do not include state normalization over the dataset as we found in our networking experiments that it dramatically reduced the performance of the resulting learned policy.
The modification to the policy improvement step is {\color{darkred}highlighted}.
We note that, with some abuse of notation, $d$ refers to the policy delay in the algorithm below, but also refers to the dimension of the critic network at other places in the manuscript.
The meaning will be clear from context.

\begin{algorithm}
\caption{TD3+BC}
\begin{algorithmic}[1]
\State Initialize critic networks $Q_{\theta_1}$, $Q_{\theta_2}$, and actor network $\pi_{\phi}$ with random parameters $\theta_1$, $\theta_2$, $\phi$
\State Initialize target networks $\theta'_1 \leftarrow \theta_1$, $\theta'_2 \leftarrow \theta_2$, $\phi' \leftarrow \phi$
\State Initialize offline dataset $\mathcal{D} = \{
(s_k, a_k, r_k, s_k')
\}_{k = 1}^K$
\For{$t = 1$ to $T$}
    \State Sample mini-batch of $N$ transitions $(s, a, r, s')$ from $\mathcal{D}$
    \State $\tilde{a} \leftarrow \pi_{\phi'}(s') + \epsilon$, $\epsilon \sim \text{clip}(\mathcal{N}(0, \tilde{\sigma}), -c, c)$
    \State $y \leftarrow r + \gamma \min_{i=1,2} Q_{\theta'_i}(s', \tilde{a})$
    \State Update critics $\theta_i \leftarrow \arg\min_{\theta_i} N^{-1} \sum (y - Q_{\theta_i}(s, a))^2$
    \If{$t~\text{mod}~d$}
        \State Update $\phi$ by the deterministic policy gradient:
        \State $\nabla_{\phi}
        J(\phi)
        =
        N^{-1}
        \sum
        \nabla_{\phi}
        \left[
        {\color{darkred}
        \lambda
        }
        Q_{\theta_1}(s, \pi_{\phi}(s))~
        {\color{darkred}
        -~
        (\pi_\phi(s) - a)^2
        }
        \right]$
        \State Update target networks:
        \State $\theta'_i \leftarrow \tau \theta_i + (1 - \tau) \theta'_i$
        \State $\phi' \leftarrow \tau \phi + (1 - \tau) \phi'$
    \EndIf
\EndFor
\end{algorithmic}
\end{algorithm}

==> sections/training_eval_details.tex <==
\section{Algorithm Training and Evaluation Details}\label{appendix.training_eval}

\mhurgent{We will fill this separately in the Supplementary Material and submit it for the Jun 12 deadline}
